Optimizing Context-Enhanced Relational Joins

Collecting data, extracting value, and combining insights from relational and context-rich multi-modal sources in data processing pipelines presents a challenge for traditional relational DBMS. While relational operators allow declarative and optimizable query specification, they are limited to data transformations unsuitable for capturing or analyzing context. On the other hand, representation learning models can map context-rich data into embeddings, allowing machine-automated context processing but requiring imperative data transformation integration with the analytical query. To bridge this dichotomy, we present a context-enhanced relational join and introduce an embedding operator composable with relational operators. This enables hybrid relational and context-rich vector data processing, with algebraic equivalences compatible with relational algebra and corresponding logical and physical optimizations. We investigate model-operator interaction with vector data processing and study the characteristics of the E-join operator. Using an example of string embeddings, we demonstrate enabling hybrid context-enhanced processing on relational join operators with vector embeddings. The importance of holistic optimization, from logical to physical, is demonstrated in an order of magnitude execution time improvement.

==> 00-abstract/main-old.tex <==
%The declarative nature of relational databases allows optimizations whose complexity is abstracted from the user.
Collecting data, extracting value, and combining insights from relational and context-rich multi-modal sources in data processing pipelines presents a challenge for traditional relational DBMS. While relational operators allow declarative and optimizable query specification, they are limited to data transformations unsuitable for capturing or analyzing context.
On the other hand, representation learning models map context-rich data into high-dimensional embeddings, allowing machine-automated context processing but requiring imperative integration with the analytical query.\\
We present context-enhanced relational operators to bridge this dichotomy and introduce an embedding operator ($\Epsilon$) composable with traditional selection and join operators. This enables hybrid relational and context-rich data processing, with algebraic equivalences compatible with relational algebra and corresponding logical and physical optimizations. We investigate model-operator interaction with high-dimensional data processing and study the characteristics of the $\Epsilon$-join similarity operator scalability over CPU and GPU. We demonstrate the importance of holistic optimization, from logical to physical, with orders of magnitude difference in execution time while enabling hybrid context-enhanced processing on relational join operator using an example of string embeddings.

==> 01-introduction/main-old.tex <==
\label{sec:introduction}
Relational databases allow declarative query specification and abstractions for logical and physical query plan optimizations. These optimizations include operator reordering via algebraic equivalences and heuristics and instantiating operators for resource-efficient and hardware-conscious execution on modern hardware, allowing ad-hoc query specification by abstracting out significant implementation details from the user and end-to-end optimization. As the main goal of relational analytical databases is to provide abstractions to large-scale processing and extraction of value from the data of interest, relational databases are designed for data types where a procedural way to process the data is possible to precisely specify, such as aggregating numerical values or processing strings with a well-specified pattern. 

Still, many data sources are unsuitable for processing in a relational database and are typically only stored serialized in binary formats. These include documents, text, images, and other data sources of increasing value, driven by the advent of the Internet and mobile devices and services such as social media. Such data has a lot of human-understandable contexts: the contents and number of objects in an image, the semantics of a string despite alternative spellings, typos, or tenses, all of which make this task impractical if not impossible to specify in traditional relational data analytics. 

On the other hand, advancements in artificial intelligence and machine learning have allowed increasingly complex machine reasoning and performance in analyzing context-rich data such as images or text. Models such as BERT~\cite{DBLP:conf/naacl/DevlinCLT19} and GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} allow natural language processing, ResNet~\cite{DBLP:conf/cvpr/HeZRS16} object localization and detection, often available as Foundation Models~\cite{DBLP:journals/corr/abs-2108-07258} that are trained on web-scale data and further customizable and re-trainable for the particular task. To use those models, analysts would instantiate the particular model, input data, and collect the output, using frameworks such as Tensorflow~\cite{abadi2016tensorflow} or Pytorch~\cite{paszke2019pytorch}, often in an isolated, task-specific setting. 

\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/Conceptual.eps}
  \caption{Problem: Model-RDBMS data analysis requires user expertise and imperative task specification.}
  \label{fig:motivation}
  \vspace{-5pt}
\end{figure}


While machine learning models can be suitable for processing context-rich, multi-modal data, deployment of such models in analytical query processing presents a manual and imperative process. Suppose an analyst wanted to analyze and extract insights from an RDBMS and use some data as input to the models as in \autoref{fig:motivation}, which may be again input to an analytical query and models in a more complex analytical processing pipeline. For example, such a use case could combine the data from social media feeds with user reviews and transaction and analytics in an online retailer case, as the data of interest and value may not necessarily be only tabular, such as in canonical TPC-H, TPC-DS, or SSB~\cite{o2007star} benchmarks.

With two independent components, RDBMS and Model, the user is back in the center of a mostly imperative program specification and data movement. This is not desirable, as a user must be an expert to fine-tune the queries, potentially perform data integration, correctly deploy and scale the queries to the hardware, orchestrate data movement, and specify the correct operator orders to avoid negatively impacting the performance. 
Decades of research and engineering in query optimization and execution engines allow hiding this complexity and is the key motivation to extend and make relational algebra compatible with emerging methods in multi-modal and context-rich processing. 

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/conceptual2.eps}
  \caption{Enabler: models embed context-rich data into common tensor representation allowing automated processing.}
  \label{fig:enabler}
\end{figure}

The key enabler of this integration is that embedding models transform the domain of context-rich data into tensors as a common intermediate data representation, allowing strictly specified operations over high dimensional vectors such as similarity or analogies, providing a method to formalize the processing of data while preserving context in neural embedding space (\autoref{fig:enabler}). A separation of concerns is established: model selection handles the multi-modality, data context, and semantics; the analytical engine optimizes and processes context-free data and tensors. 

Still, two components need to communicate and be tightly integrated, and we investigate the model-operator interaction and optimizations through the example of tensor-based similarity join processing using word embedding model~\cite{DBLP:journals/tacl/BojanowskiGJM17}, and:
%Our contributions:
\begin{itemize}
    \item Motivate the need for context-enhanced operators in \autoref{sec:motivation}, and introduce the model-operator interaction and formalize extended relational operators in \autoref{sec:model-operator-interaction},
    \item Propose a cost model, logical optimizations, and an alternative tensor formulation for parallel execution of relational operators for processing neural embeddings in \autoref{sec:logical-optimization},
    \item Recommend physical and hardware optimizations in \autoref{sec:physical-optimization}, and evaluate the operator implementation and characteristics on CPU and GPU in \autoref{sec:evaluation} that impact the execution time over orders of magnitude, showing the importance of logical and physical optimizations of enhanced relational operators.  
\end{itemize}

%While we have systems for vector data management, we are intersted in systems that combine relational with vector data. Simple example are strings in the databases, on which we focus in this paper. 
%while optimizable and declarative algebra for 

%FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17} Word2Vec~\cite{DBLP:journals/corr/abs-1301-3781}

%Many data sources, need for unification, example.

%While there exist efficient model deployment platforms that can perform inference, this would leave user to perform consolidation on their own. Integration of the system, physical and logical optimizations, hardware management which are both time consuming, error prone, and may lead to suboptimal performance. 



%\autoref{sec:introduction}




==> 02-motivation/main-old.tex <==
\label{sec:motivation}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/conceptual_solution.eps}
  \caption{Goal: Models and operators are equal declarative data transformation primitives amenable to optimizations.} %  Solution - interface, logical, and physical optimizations
  \label{fig:motivation_solution}
  \vspace{-5pt}
\end{figure}

Data management systems support and simplify data processing with rich research and systems contributions and features such as transactions and concurrency control~\cite{zhang21, DBLP:conf/icde/KemperN11}, auto-tuning~\cite{pavlo17}, hardware-conscious implementations~\cite{DBLP:journals/pvldb/Neumann11, DBLP:journals/pvldb/ChrysogelosKAA19, DBLP:conf/cidr/NeumannF20, DBLP:journals/pvldb/KerstenLKNPB18, DBLP:conf/icde/ZukowskiWB12}, corresponding data structures~\cite{DBLP:conf/sigmod/IdreosZHKG18}, and query optimization with declarative interfaces to abstract out the system complexity from the end-user.
To analyze and reason about multi-modal and context-rich data using machine learning, there are mature systems such as Tensorflow~\cite{abadi2016tensorflow} or PyTorch~\cite{paszke2019pytorch} that support model training and inference.

Manual intermediate orchestration and system integration would be required to combine and analyze multi-modal and context-rich data, involving different systems, data sources, and operator reimplementation on various hardware targets. While users may have efficient engines for different data sources (\autoref{fig:motivation}), the intermediate orchestration resembles that of federated database systems~\cite{10.1145/96602.96604}. 
While there has been prior work to integrate model inference and learning with analytical engines~\cite{DBLP:conf/icde/LinWZDLC22, DBLP:journals/pvldb/HellersteinRSWFGNWFLK12}, our goal is complementary as we focus on how we can extend the functionality and better optimize relational operators that serve as an interface and standalone operations between a relational engine and an embedding model, as illustrated in \autoref{fig:motivation_solution}. Similarly, our goal is to expose co-optimization opportunities at logical, physical, and implementation levels, and expose fine-grained interactions between data structures and algorithms, particularly in an example of a join operator.

While there are index structures designed to store, maintain, and perform similarity search over tensors~\cite{DBLP:conf/sigmod/WangYGJXLWGLXYY21, DBLP:journals/tbd/JohnsonDJ21}, as well as a vector database systems~\cite{DBLP:conf/sigmod/WangYGJXLWGLXYY21}, they are typically limited to search operations and limited functionality and do not support operations such as joins or co-optimization with the analytical operators and the execution plan of the RDBMS. Still, they are important components for building a data management system that supports tensor data processing. Similarly, recent work has formulated traditional relational processing over tensors~\cite{DBLP:journals/corr/abs-2211-02753}, where tensor processing platforms are used as analytical RDBMS to benefit from existing implementation over heterogeneous hardware while paying for data transformation and standalone implementation. 

We investigate how to extend traditional relational data management systems to support model-driven context with minimal system intrusions and building on top of the existing systems using existing judiciously modified abstractions.


%% HOLISTIC OPTIMIZATION
\subsection{Holistic Optimization}\label{ssec:holistic-optimization}

Without loss of generality, suppose the data of interest are strings and dates stored in an RDBMS. Generally, one can consider other context-rich formats stored as binary objects with other relational data. To allow semantic similarity operations, such as matching strings that are synonyms, have misspellings, or different tenses, word embedding models such as FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17} transform strings into vectors which are then comparable using cosine distance. Note that the model can be trained and adapted for different datasets to adjust the notion of similarity. We are interested in joining two tables over strings, where a condition over dates exists, making the queries selective on both tables. 

Normally, RDBMS could optimize and execute a query over regex-like string operations. Still, using a model and embeddings, interaction needs to be specified and optimized logically, physically, and depending on the target runtime hardware.
In a declarative setting, query specification requires embedding model information and the join condition expression, and the selectivity information from the relational column needs to propagate before the embeddings. Otherwise, the whole interaction may result in the user eagerly materializing all the data as in~\autoref{fig:motivation}, performing expensive embedding, and only then filtering. In more complex cases and ad-hoc queries, imperative specification and optimization are increasingly difficult.

Even with a declarative query with a logical plan with correct selectivities and operator orders, the word embedding model must interact with a join operator. Physical optimization must address this interaction and account for the tensor data format and the expressions suitable for comparing high-dimensional data. For example, while an equi-join over tensors could be implemented as a hash-join, more practical embedding comparisons, such as cosine distance, require algorithms such as nested-loop join for pair-wise comparisons and consider the join, operation, and model data structure access patterns in the algorithm and cost model.

For holistic optimization (\autoref{fig:motivation_solution}), starting from declarative specification through logical and physical optimization, and finally, hardware specialization to allow efficient execution on different physical devices such as CPUs or GPUs. Relational operators were typically designed and optimized for single-dimensional numerical data and judicious use of caches and memory hierarchy. A 100-dimensional tensor embedding will change the caching and execution patterns of traditional algorithms, and model embedding can incur computational or data access costs at a critical path of execution. Designing hardware-conscious algorithms represents a direction driven by novel model-database interactions.

Some tasks that are challenging research questions are not in the scope of this paper. Firstly, we do not exhaustively evaluate every model and operator interaction, such as selection or group-by operators. Secondly, many possible embedding models exist for multi-modal data to evaluate, tune, and provide automatic selection methods~\cite{2ab49deedb854506850bf44e67aa808c} for different cases. Future work will explore open topics such as data layouts, storage, indexing, caching, resource scheduling, and cardinality estimation with embedding models running over a multi-modal, federated data management system. Still, the abstractions we present in this paper and join operator cost analysis using word embeddings and optimizations are applicable in a more general setting, bringing forward systematic analysis and optimization of context-enhanced relational operators with embedding models. 

%in the most general case, model-operator interaction and online transformation, but could be cached. online case since it is typically expensive, and we consider this as a separate cost, breaking down the opaque box of the model for co-optimizations.
%tensors are just one more data type, invisible to relational engines. we can build on top of them.
%data lakes and process only what is necessary~\cite{10.14778/3352063.3352116}
% maybe give an example related to how models and RDBMS may be used - and the effects of it with reference to ICDE vision paper~\cite{sanca2022analytical}
%Combining multiple systems and operations can be both tedious, scheduling, performance, and optimization. We propose extending relational operators with context so we can benefit from existing systems. UDF potential solution.

%As simple as selecting a model and how interact with other data, fully independent of format etc
%other embeddings etc, how does this generalize.


\subsection{Extended Functionality}

The separation of concerns via model-driven embeddings along the relational operators allows data that was previously opaque to the relational data management system to be mapped into the embedding domain (and back), which allows operations over vectors and tensors such as semantic similarity using cosine distance or other vector arithmetic operations, such as finding word analogies. We describe potential use cases for such context-extended relational data management systems.

%% SIMILARITY OPERATIONS
%\subsection{Semantic-Based Similarity Operations}\label{ssec:semantic}
\subsubsection{Semantic-Based Similarity Operations}\label{ssec:semantic}

Instead of having a human-in-the-loop or an expert system that performs dictionary-based or hard-coded rule-based similarity operations, neural embeddings allow automating the similarity operations over many data types. In practice, embedding the data into a common tensor representation and allowing such similarity search or joins replaces manual similarity specification with distance-based specification, such as cosine distance between the embedded vectors. The models fine-tune the functionality and context. After embedding the data and providing operators and expressions over tensors such as cosine distance, model-independent operations can be combined with the rest of the relational query plan.


%% ONLINE DATA INTEGRATION
%\subsection{Online Data Integration}\label{ssec:data-cleaning}
\subsubsection{Online Data Cleaning}\label{ssec:data-cleaning}

Strings or other context-rich data can be dirty or have rich semantics.
If we consider words or sentences, they may have misspellings, alternative spellings, synonyms, or different tenses that all have the same meaning.
Specifying all the rules to unify context is error-prone and difficult, while word embeddings can encompass such similarity using representation learning. Therefore, such operators can process such data on the fly without prior cleaning and only the data of interest, relying on embeddings and specified similarity thresholds for data integration and potentially performing post-verification steps.


%% MULTI-MODAL DATA PROCESSING
\subsubsection{Multi-Modal Data Processing}\label{ssec:multi-modal-data}

The data context is opaque to the execution engine, while the model selection and parameters give context and transform the data. By processing context-free tensors, relational engines provide a common framework for multi-modal data. Of course, such operations are not all-encompassing but provide a step towards unifying relational with model-driven data processing under a declarative and optimizable pipeline.\\


\paragraph{Takeaway}
Neural embedding models transform the context-rich, multi-modal data into a common (per-model) tensor representation space. From the perspective of declarative relational processing, models provide separation between data semantics and context-less tensors as a model-parametrized projection operator. From there, relational operators perform operations such as cosine distance or vector transformations over tensors, amenable to query optimization via common abstractions and cost models that include model-operator interactions and physical optimizations aware of tensors and new computation and data access patterns that can be specialized for different hardware runtimes. We analyze these behaviors and propose solutions aware of the new design space.


==> 03-model-operator-interaction/main-old.tex <==
\label{sec:model-operator-interaction}

We propose a relational operator extension to declaratively process context-rich data stored along traditional relational data, such as strings and text, that may be associated with numerical or date attributes. This enhancement stems from the fact that the contextual data may need to be transformed and processed differently. However, compatibility with relational algebra and optimizations for processing purely relational data is required. Instead of using separate systems and manually orchestrating the data movement for processing using external programs or opaque UDFs, we propose a set of operations based on embedding the original data amenable to traditional query optimization.

%%%%%%%%%%%%%%%%%%%
\subsection{Neural Embeddings}  \label{ssec:neur-emb}

There have been significant efforts to enable machine-automated understanding of context-rich data. The key idea behind neural embeddings is that the model ($\mu$) learns how to transform the input data domain into high-dimensional vector space (\autoref{fig:enabler}), where relationships between the data can be expressed using linear algebra expressions over vectors. Embeddings ($\Epsilon$) take a human-understandable context-rich domain and map it into a machine-operable high dimensional vector (tensor) space. 

Neural embeddings and representation learning are rich and active research fields in machine learning. Images can be embedded with models such as ResNet~\cite{DBLP:conf/cvpr/HeZRS16}, audio with PANNss~\cite{DBLP:journals/taslp/KongCIWWP20}, and text with Bert~\cite{DBLP:conf/naacl/DevlinCLT19}, word2Vec~\cite{DBLP:journals/corr/abs-1301-3781}, FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17, DBLP:conf/naacl/EdizelPBFGS19}. Foundation Models~\cite{DBLP:journals/corr/abs-2108-07258} offer an increasingly flexible way to specialize large models to a particular use case. It is important to mention those models can be tuned, as they learn representations from the training dataset through transfer learning~\cite{DBLP:conf/naacl/QiSFPN18} (e.g., starting from one of the foundation models) or re-training. In this work, we focus on and experiment with string embedding models. However, as embeddings are generally high-dimensional vectors, once in the embedding domain, the processing of this data is model- and input-data-type-agnostic, and the same principles and optimizations hold.

Processing embedded data allows automating semantic similarity using cosine similarity (or another distance) between the vectors. More complex relationships in the vector space are possible, such as analogies, such as country capitals \texttt{(Switzerland $\rightarrow$ Bern), (Greece $\rightarrow$ \textbf{Athens})}. The equations below outline definitions of cosine similarity over vectors and matrices, and we will use them heavily in execution optimization phases.

\begin{equation}
\tag{Cosine Similarity}
\label{eq:cosine-sim}
cos(\theta) = \frac{A \cdot B}{\lVert A \rVert\lVert B \rVert} = \frac{\sum\limits_{i=1}^{n}A_i B_i}{\sqrt{\sum\limits_{i=1}^{n}A_i^{2}}\sqrt{\sum\limits_{i=1}^{n}B_i^{2}}}
\end{equation}


\begin{equation}
    \tag{Vector-Vector}
    \label{eq:vec-vec}
    \frac{\mathbf{a}^{(1,d)} \cdot \mathbf{b}^{(1,d)}}{\lVert \mathbf{a} \rVert\lVert \mathbf{b} \rVert} = \frac{\sum\limits_{i=1}^{d}a_i b_i}{\sqrt{\sum\limits_{i=1}^{d}b_i^{2}}\sqrt{\sum\limits_{i=1}^{d}b_i^{2}}}
\end{equation}

\begin{equation}
    \tag{Vector-Matrix}
    \label{eq:vec-mat}
    \frac{\mathbf{a}^{(1,d)} \cdot \mathbf{B}^{(m,d)}}{\lVert \mathbf{a} \rVert\lVert \mathbf{B} \rVert} 
    = \left[\frac{\mathbf{a} \cdot \mathbf{b}_i}{\lVert \mathbf{a} \rVert\lVert \mathbf{b}_i \rVert}\right]_{i=0}^{m}
\end{equation}

\begin{equation}
    \tag{Matrix-Matrix}
    \label{eq:mat-mat}
    \frac{\mathbf{A}^{(n,d)} \cdot \mathbf{B}^{(m,d)}}{\lVert \mathbf{A} \rVert\lVert \mathbf{B} \rVert} 
    %= \left[\frac{\mathbf{a}_i \cdot \mathbf{B}}{\lVert \mathbf{a}_i \rVert\lVert \mathbf{B} \rVert}\right]_{i=0}^{n}
    = \left[\left[\frac{\mathbf{a}_i \cdot \mathbf{b}_j}{\lVert \mathbf{a}_i \rVert\lVert \mathbf{b}_j \rVert}\right]_{i=0}^{n}\right]_{j=0}^{m}
\end{equation}



%%%%%%%%%%%%%%%%%%%%
\subsection{Model-Operator Interaction}

We focus on context awareness over strings so that common mistakes or semantically similar words are automatically captured. Rather than imposing user to strictly specify the rules for string similarity or clean the data ahead of time, we enable words such as (\texttt{barbecue}, \texttt{barbecues}, \texttt{bbq}, \texttt{barbicue}, \texttt{grilling}) that have similar semantics, to automatically be used with relational operator predicates without prior user intervention. The user should only specify the embedding model and a threshold distance parameter over cosine similarity calculation (\autoref{eq:cosine-sim}). Instead of comparing two strings in their original domain, they are embedded. If the cosine similarity $cos(\theta)$ is larger than the specified threshold, the two strings are similar and should be matched. This avoids manual string processing and combining techniques, such as Locality Sensitive Hashing, individually limited to capturing only features such as misspellings.

In this work, we use FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17, DBLP:conf/naacl/EdizelPBFGS19} as a model ($\mu$) for word embeddings, which has the desirable properties that it can be trained and adapted to the context, it supports out of vocabulary word embedding and is resilient to misspellings. A context-aware operator is supplemented with an embedding model. In this case, when an operator receives strings, it embeds them using FastText and then performs the requested processing in the vector domain. 
This interaction opens up design and optimization choices, such as how to mask or minimize the cost of embedding/model and overlap it with operator execution. 
We capture this interaction through relational algebra (\autoref{ssec:rel-ops}) and a cost model (\autoref{sec:logical-optimization}) to allow holistic integration with the remainder of the query plan.


%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relational Operators and Algebra} \label{ssec:rel-ops}

We introduce the embedding operator ($\Epsilon$) using a model ($\mu$), and relational algebra equivalences over selection ($\sigma$) and $\theta$-join ($\bowtie_{\theta}$) operations, compatible with traditional relational algebra.

\subsubsection{Selection}% - $\sigma$}

The selection operation applies predicate $\theta$ over input tuples and returns only the tuples that satisfy the condition.

\begin{equation}
\tag{Selection with predicate $\theta$}
\sigma_{\theta}(R) = \{ t \in R,\ \theta(t) \}
\end{equation}

To change the domain of input data, we allow mapping the input tuples (or a projection over the tuples for simple notation) using a model ($\mu$) into vector space using embedding ($\Epsilon$) operation. 

\begin{equation}
\tag{Embedding with model $\mu$}
\Epsilon_{\mu}(R) = \{ t \in R,\ t \mapsto \mu(t) \}
\end{equation}

For completeness and decoding of the embeddings and retrieving the context-rich data, an inverse operation $\Epsilon^{-1}$ should also be defined, which is the standard component of encoder-decoder architectures, and semantically correct only for the same model $\mu$.

\begin{equation}
\label{eq:decode}
\tag{Decoding with model $\mu$}
\Epsilon^{-1}_{\mu}(\Epsilon_{\mu}(R)) = R
\end{equation}

Combining embedding with selection allows the processing of tuples with a mixture of data formats. Some attributes may have traditional relational predicates, and some may require embedding and predicates using different metrics (such as cosine distance). Predicate pushdown and operation reordering can happen as soon as the attributes that predicates operate over are available.

\begin{equation}
\tag{$\Epsilon$-Selection}
\sigma_{\Epsilon, \mu, \theta}(R) 
\Leftrightarrow 
\sigma_{\theta}(\Epsilon_{\mu}(R))
\Leftrightarrow 
\sigma_{\theta_{\Epsilon}}(\Epsilon_{\mu}(\sigma_{\theta_{R}}(R))))
\end{equation}


\subsubsection{Join}% - $\bowtie$}

The join operation takes two relations and joins them over specified attributes using specified predicate conditions ($\theta$-join).

\begin{equation}
\tag{Cartesian Product}
R \times S = \{ (r,s),\ r \in R \wedge s \in S \}
\end{equation}

Joins are amenable to predicate pushdowns and reordering.

\begin{equation}
\tag{$\theta$-Join Generalization}
R \bowtie_{\theta} S 
\Leftrightarrow 
\sigma_{\theta}(R \times S)  
\end{equation}

We introduce embeddings to the generalized join definition and provide equivalences. Embeddings can be observed as a special projection operation that changes the domain.

\begin{equation}
\tag{$\Epsilon$-$\theta$-Join}
\begin{split}
R \bowtie_{\Epsilon, \mu, \theta} S 
\Leftrightarrow 
\sigma_{\Epsilon, \mu, \theta}(R \times S)\\
\Leftrightarrow\\
\sigma_{\theta}(\Epsilon_{\mu}(R) \times \Epsilon_{\mu}(S))
\Leftrightarrow
\Epsilon_{\mu}(R) \bowtie_{\theta} \Epsilon_{\mu}(S) 
\end{split}
\end{equation}

%\subsubsection{Grouping}% - $\Gamma$}
%$\Gamma$

Conversely, decoding the embeddings into their original domain is possible across the plan (\autoref{eq:decode}).\\

\paragraph{Takeaway}
We formulate the context-enhanced operators by extending relational operators and algebra to allow declarative integration of embedding models with relational engines and optimizers. A hybrid setting enables declarative and systematic logical and physical optimizations while providing semantic awareness using embeddings to separate concerns between models and engines.



==> 04-logical-optimization/main-old.tex <==
\label{sec:logical-optimization}

\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/Matrix1.eps}
  \caption{Matrix formulation of $\Epsilon$-join allows scalable and cache-efficient execution over high-dimensional embeddings.}
  \label{fig:tensor}
\end{figure*}

Starting from the extended algebra and operators, we present the logical optimization driven by model-operator interaction and tensors as a common intermediate data representation. In contrast to traditional optimizations and relational operator cost models, the two factors are different. First, since models may be on the critical path of execution, model embedding data access or computation time must be considered in addition to the relational operator's data access and processing cost. Second, embeddings change the data domain from traditionally \textit{atomic} data types (prescribed by the 1$^{st}$ normal form) into dense high-dimensional vectors, which could benefit from optimizations in the domain of linear algebra. Still, regarding the 1$^{st}$ normal form, embeddings are not structured data but should be observed and processed atomically.

This changes the cost model and impacts the known characteristics of algorithms. For example, suppose an embedding is a 100-D vector. In that case, the cost of data movement and cache locality characteristics (spatial and temporal) are changed and must be evaluated in conjunction with the model's behavior and internal data structures.

\subsection{Cost Model}

%\begin{equation}
%    \tag{Selection Cost}
%    Cost(\sigma_{\theta}(R)) = Access(|R|) + Compute(\theta(|R|)) 
%\end{equation}

We outline the abstract cost model for the context-enhanced selection and join operations. For joins, we investigate the nested-loop join strategy. 
It is important to note that we evaluate exact algorithms in our study. Since the distance we use is cosine similarity, hash-based approaches would yield approximate solutions similar to Locality Sensitive Hashing. 
Of course, if we were to use equi-joins, it would be possible to use traditional hash-joins, but there would be no benefit from using embeddings.
Still, nested loop joins are a good fit as they can be formulated with good cache-locality, an important performance factor (\autoref{sec:evaluation}) that does not incur random access over high dimensional data as every vector needs to be pair-wise compared using cosine distance.

Similarly, there are index structures that store and enable efficient search of high-dimensional data~\cite{DBLP:journals/tbd/JohnsonDJ21}, providing a direction for evaluating the performance of index-join implementations. A detailed comparison and performance evaluation between different exact, approximate, and index-based $\Epsilon$-join strategies is a topic of future work. For now, we outline the cost model for selection and join below, where $R$ and $S$ are relations, $|R|$ is the cardinality of relation $R$, $A$ represents the data access cost, $M$ represents the model cost, and $C$ is the computation cost.

Selection is an operation where input data is scanned, embedded, and the condition is applied over every input tuple, where each tuple incurs access, computation, and model cost:
\begin{equation}
    \tag{$\Epsilon$-Selection Cost}
    Cost(\sigma_{\Epsilon, \mu, \theta}(R)) = |R| \cdot (A + M + C) 
\end{equation}

Nested-Loop Join (NLJ) operation scans both relations and performs pair-wise condition comparisons. In a naive implementation without considering model-relational interaction, model access would be performed per-processed tuple, which incurs quadratic model access cost. Considering that embedding models are computationally expensive, the following cost model is suboptimal:
\begin{equation}
    \label{nlj-naive}
    \tag{$\Epsilon$-NL Join Cost}
    Cost(R \bowtie_{\Epsilon, \mu, \theta} S) = |R| \cdot |S| \cdot (A + M + C)
\end{equation}

Instead, by considering the characteristics of the nested-loop join, we observe that tuple embedding needs to happen only once per tuple from both relations. This can be performed as a precursor to the join operation or as lazy embedding and data materialization. By observing this behavior, the join results in a linear model cost:
\begin{equation}
    \label{nlj-prefetch}
    \tag{$\Epsilon$-NLJ Prefetch Optimization}
    Cost(R \bowtie_{\Epsilon, \mu, \theta} S) = |R| \cdot |S| \cdot (A + C) + (|R| + |S|) \cdot M 
\end{equation}

This optimization is significant, as the model cost can span from random access to a lookup table (several times slower than sequential scan) to expensive computations over deep neural networks (data transfer and computation). 
From another perspective, if machine learning models are used as-a-service and paid for per embedding, this cost model conversely results in monetary savings compared to the potential suboptimal, manual implementation.
Expressing embeddings as relational operator extensions allows logical optimization to occur in conjunction with other operators in the hybrid relational-embedding pipeline (selection pushdown, join reordering), such that the cardinality of the most costly part of the query plan will be reduced without explicit user intervention or knowledge about specific interactions given a relational operator.

%\subsection{Rule- and Cost-Based Optimization}
%Similar like relational algebra, explain briefly.
%Prefetch. Model cost, data structures.


%%%%

\subsection{Tensor Join Formulation}

Since the computation of context-enhanced operators happens over dense high-dimensional embedding vectors, following the vector and matrix definitions of cosine distance in \autoref{ssec:neur-emb}, we present the tensor formulation of the dot product. It is important to notice that cosine similarity is equivalent to the dot product in case input vectors are normalized.

The tensor formulation allows reasoning about the potential decomposition of the problem for parallel and cache-efficient execution beyond data parallelism. This allows using efficient and well-studied matrix-based algorithms for linear algebra in addition to the traditional relational algorithms. We present the block-matrix decomposition of the problem~\cite{IMM2012-03274}. 

\input{04-logical-optimization/tensor_formulation}

Given a $(|R| \times dim)$ matrix $\mathbf{R}$ with $t$ row partitions and $d$ column partitions, and a $(dim \times |S|)$ matrix $\mathbf{S}$ with $d$ row partitions and $v$ column partitions that are compatible with the partitions of $\mathbf{R}$, dot product $\mathbf{D} = \mathbf{R}\mathbf{S}$ can be formed block-wise, yielding $\mathbf{D}$ as a $(|R| \times |S|)$ matrix with $t$ row partitions and $v$ column partitions.
We consider $\mathbf{S}$ to be already transposed if the initial data layout is as of $\mathbf{R}$; in other words, matrices $\mathbf{R}$ and $\mathbf{S}$ are compatible.

In particular, we partition the data along the tuple lines, not the dimensions, as illustrated in \autoref{fig:tensor} \textcircled{1}. Transforming the initial Nested-Loop Join into Tensor formulation allows matrix multiplication algorithms to achieve better cache utilization of high-dimensional data, with well-understood parallelization using block-matrix decomposition. 

This is compatible with and extends recent research on formulating relational operators for tensor processing runtimes~\cite{DBLP:journals/pvldb/HeNBSSPCCKI22}. 
The cache is utilized better as, in contrast to NLJ, a matrix block (several vectors) can remain in the cache and be reused over many operations. 
Block-matrix partitioning allows for defining the processing granularity, which is significant when memory footprint needs to be constrained, as in GPU processing, allowing fine control of both the transfer and processing granularity of cosine-distance-based similarity operations, all while reducing redundant data transfers. 
As in \autoref{fig:tensor} \textcircled{2}, to map back to corresponding tuple pairs that satisfy the \texttt{threshold} condition, it is sufficient to maintain the starting offsets of input relation partitions, so the result set constitutes a potentially sparse matrix of pairs that represent matrix batch offsets.
This result can be considered as using late materialization, and while sparse, it is more compact as tuples of offsets represent tensors. This is increasingly important when using devices with limited memory, such as GPUs, designed for tensor computations and can return the results to the CPU faster via interconnects in this representation.\\

\paragraph{Takeaway}
Formulating the cost model and alternative equivalent execution plans using linear algebra allows tuning the algorithms to the cost model and execution environment parameters, as high-dimensional vectors and model processing introduce data access, caching, and processing overheads different from traditional relational operators that often process only single-dimensional data.


==> 05-physical-optimization/main-old.tex <==
\label{sec:physical-optimization}
Modern data management systems are designed and optimized to efficiently utilize available hardware resources~\cite{DBLP:journals/pvldb/ChrysogelosKAA19, DBLP:conf/icde/ZukowskiWB12, DBLP:journals/pvldb/Neumann11}. Equally, machine learning frameworks and vector management systems are designed with physical optimizations to allow fast and efficient execution~\cite{abadi2016tensorflow, paszke2019pytorch, DBLP:conf/sigmod/WangYGJXLWGLXYY21, DBLP:journals/tbd/JohnsonDJ21}.

Therefore, we consider modern hardware and accelerators in the landscape of physical optimizations. We design our operators with in-memory execution characteristics in mind. To consume the available memory bandwidth, multi-threaded execution is necessary. As GPUs have become commonplace for ML and data management acceleration, we consider their characteristics and interconnect transfer optimization. We equally consider optimizations driven by the ML community, such as fast matrix operations and half-precision computation (when natively supported by hardware)~\cite{rodriguez2018lower}.

\subsection{Data-Parallel Execution}

To benefit from many-core architectures and massively-parallel GPUs, we outline the parallelization and hardware-conscious optimizations of the join algorithm. In contrast to the traditional Nested-Loop Join (NLJ) that allows exact cosine-distance-based joins, high-dimensional embedding vectors take up more space in the cache hierarchy. 
Consider a 32KB L1 cache, and we operate over 4-byte values. 
Using a 100-dimensional embedding vector, the L1 cache can store only 80 values, in contrast to 8000 for the single-dimensional data type. 
This necessitates cache-efficient implementation to benefit from the memory hierarchy.
Furthermore, computing cosine distance over vectors requires more computation cycles than simply performing the regular value-based operation.
Thus, judicious use of hardware resources is necessary to speed up data access and computation.

\subsubsection{Data-parallelization strategies}
Nested-Loop Join can be parallelized by partitioning the input relations and using a heuristic of keeping the smaller relation inside the inner loop to improve data and cache locality. This is a traditional and well-known NLJ algorithm implementation and optimization. 
In addition, we propose using the matrix (tensor) formulation (\autoref{fig:tensor}) as an alternative to NLJ. 
As matrix multiplication to obtain a dot product and normalize the vectors is embarrassingly parallel, in addition to having fine-grained control over partition size. 
In contrast to NLJ, matrix multiplication over dense vectors has improved cache locality~\cite{DBLP:journals/toms/GotoG08, DBLP:conf/ipps/SmithGSHZ14}, improving the use of the memory hierarchy in the presence of high-dimensional data, and using efficient matrix multiplication algorithms and linear-algebra frameworks.

\subsubsection{SIMD Vectorization}
Executing linear algebra operations such as cosine distance over dense vectors is compute-intensive and involves repeated operations over every vector embedding element. 
Since the operations such as sum are repeated over every element of the logical vector, it is a natural fit for using single-instruction multiple-data instructions (SIMD). 
We use SIMD vectorization supported by hardware to speed up the arithmetic operations using fewer processing cycles using specialized registers and compute units, as illustrated in \autoref{fig:simd}, in conjunction with data-parallel partitioning for multi-core operator execution.

\begin{figure}
  \centering
  \includegraphics[width=0.6\linewidth]{figures/SIMD.eps}
  \caption{High-dimensional vectors are suitable for SIMD.}
  \label{fig:simd}
  \vspace{-5pt}
\end{figure}



\subsection{Hardware Acceleration: CPU and GPU}

With multi-core CPU architectures and GPUs becoming commonplace for modern data analytics and machine learning environments, we outline specific hardware acceleration opportunities and characteristics we have considered for the performance study. We evaluate in-memory execution and defer caching and storage hierarchy research for future work.

\subsubsection{CPUs} benefit from data locality and fast main memory access. Traditionally, they are general-purpose compute units designed to process full-precision data types (e.g., 32-bit, 64-bit). They typically support SIMD, such as with Intel AVX instructions. Recent AVX-512~\cite{intelavx512fp16} instruction set has introduced hardware support for half-precision data types, which allows processing up to 32 16-bit floating point numbers in a SIMD register. Furthermore, to support typical machine learning workloads, beyond providing hardware support for half-precision data types, CPUs such as 4th generation Intel Scalable Xeon Processors introduced specialized instruction sets (AMX) to accelerate matrix computations.~\cite{nassif2022sapphire}. Still, due to general-purpose architecture, specialized accelerators such as GPUs have gained prominence in ML and recent database systems~\cite{DBLP:journals/pvldb/ChrysogelosKAA19}.

\subsubsection{GPUs} benefit from massive parallelism and optimizations that target linear algebra, driven by the need for ML-model training and inference. 
Furthermore, GPUs often have specialized compute units such as tensor cores~\cite{DBLP:conf/ipps/MarkidisCLPV18} that further accelerate linear algebra operations over vectors.
GPUs have significantly higher internal memory bandwidth than CPUs, but the memory is limited in capacity, requiring data partitioning considerations such as using \ref{eq:decomposition}.
Furthermore, GPUs require data transfer from the main memory over the interconnect, where considerations about streaming and retrieving the data, as the late materialization join result retrieval in \autoref{fig:tensor} \textcircled{2} are important. 
Due to hardware specialization, GPUs better fit context-enhanced operators, especially the matrix join algorithm formulation.

\subsubsection{Data Type Precision, Embedding Size} While data analytics typically prescribe computation over the specified data types, ML-community is familiar with using mixed-precision and half-precision data types~\cite{DBLP:conf/iclr/MicikeviciusNAD18}. This allows trading some accuracy for processing efficiency. Specialized hardware support exists in some CPUs and GPUs, driven mainly by model inference use cases, compatible with linear algebra acceleration. 
On the other hand, neural embedding models often have parametrized embedding vector sizes or otherwise allow for dimension reduction. This allows tuning the expected model embedding accuracy for memory, data access, and processing time. Let us again consider the 32KB L1 cache size case, with vector dimensionality of 100 and 500 elements, stored as either 32-bit floating point (FP32), or 64-bit double precision floating points (FP64). The cache capacity varies from 80 to 8 vector elements, reducing the throughput of SIMD operations with fixed-width register sizes. \\

\paragraph{Takeaway}
The physical operator design landscape encompasses both implementation and hardware device characteristics-based decisions. 
Model-operator interactions only enrich the design space.
High-dimensional data contributes to reduced capacity of the memory hierarchy in comparison to common atomic data types found in relational data processing and requires rethinking cache-local implementations.
Per-tuple compute significantly increased, shifting the bottleneck from traditionally memory-bound analytics to more compute-heavy operations, which invites the use of specialized hardware accelerators and hardware-conscious algorithms.


==> 06-evaluation/main-old.tex <==
\label{sec:evaluation}

We briefly demonstrate the functionality of context-enhanced relational operators using word embeddings and next study the performance and impact of logical and physical optimizations on CPU and GPU runtimes.

\subsection{Functionality with Word Embeddings}
In our study, we use the example of word embeddings that transform input strings into high-dimensional vectors. We show the context-awareness functionality that word embeddings allow and note that embedding models can be fine-tuned and replaced to support different notions of similarity. Conversely, there are embedding models to support different data modalities, which is out of the scope of our paper. Still, the intermediate data representation of an embedding is a context-free tensor where our analysis is applicable.

\paragraph{Embedding Model}
We use FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17} word embedding model, which allows out-of-vocabulary embeddings and retrieving in-vocabulary embeddings from a hash-table structure. 

\paragraph{Dataset}
We train a 100-dimension embedding model over a subset of Wikipedia dataset~\cite{wiki}, cleaned of stopwords.
We use a subset of 1M strings from the dataset to test the similarity using the model.




\begin{table}[hb]% h asks to places the floating element [h]ere.
  \caption{Semantic Matching using FastText trained on Wikipedia dataset, 100-D embeddings, sample words.}
  \label{tab:sem_example}
  \begin{tabularx}{\linewidth}{p{0.12\linewidth}  p{0.82\linewidth} }
    \toprule
    Word & Top-15 Model Matches\\
    \midrule
    dbms & rdbms, nosql, dbmss, postgresql, rdbmss, sql, dbmses, sqlite, dataflow, ordbms, oodbms, couchdb, mysql, ldap, oltp\\
    \hline
    postgres & postgre, postgresql, openvt, dbms, rdbmss, sqlite, dbmss, odbc, backend, rdbms, rdbmses, postgis, openvp, couchdb, mysql\\
    \hline
    animal & animals, felines, human, bovines, equines, dogs, nonhuman, ferrets, rabbits, chickens, anthropods, bovine, anthropod, mammal, equine\\
    \hline
     dog & dogs, poodle, doberman, sheepdog, puppies, dachshund, hound, bullmastiff, retriever, pinschers, dobermans, puppy, bullmastiffs, chickenhound, dachshunds\\
    \hline
    clothes & dresses, clothing, garments, underwear, bedclothes, undergarments, towels, underwears, scarves, shoes, nightgowns, clothings, bathrobes, underclothes\\
  \bottomrule
\end{tabularx}
\end{table}

We want to show the Top-15 nearest vectors to sample words as the strings are embedded into a high-dimensional vector space. We then decode the vectors back into string and present sample semantic matches in \autoref{tab:sem_example}. The model has learned semantics and context from the Wikipedia dataset. To fine-tune the model, it is possible to specialize the embedding models with other domain-specific datasets. However, we limit our study to a proof of concept using word embeddings with the FastText model. The principle of managing and producing embeddings remains the same.

It is important to mention that models allow automated semantic matching, and the strings are not materialized or retrieved during operations in an intermediate step. Instead, the computation fully happens on embedded data, and only positive matches are retrieved. It is possible to decode the embeddings, for example, based on their offset in the input relation and processing the embedding using standard encoder-decoder model architecture.

Furthermore, we can notice that this model detected synonyms, semantic and related matches, and plural forms of the words without external user specification. The only parameter in the case of a join with cosine distance would be a single threshold parameter. This allows relational operators normally operating over sample strings (i.e., Word column in \autoref{tab:sem_example}) to perform matches with strings on the right in the embedding domain without humans in the loop or experts that would create and specify strict rules.


%More expensive models, online, bert, future work! no standardized benchmark, but the benefit is recognized, and we do not claim the benefits of embeddings, but formalize how they should interact. still, we provide a preview, also available for other multi-modal data. Open source and closed-source models, cost analysis. Dimensions can also change, but usually vary from X to Y, but the main benefit is that the data type itself is immutable (tensors), therefore the analysis.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CPU
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% alternatively just have performance and subsubsections
\subsection{CPU Performance}
We first evaluate the impact of logical and physical optimizations on the execution time using CPUs.

\paragraph{System} we implement our benchmarks in a standalone system in C++ using GCC 12.1.0 compiler, that allows native FP16 support. Tensor formulation benchmarks are implemented using TensorFlow 2.11.0 as a framework for high-performance linear algebra, optimized with Intel oneAPI Deep Neural Network Library to use Intel AVX instructions for SIMD execution.

\paragraph{Hardware Setup} We run the end-to-end and scalability experiments on two-socket Intel Xeon Gold 5118 CPU (2 x 12-core, 48 threads) and 384GB of RAM. To evaluate the impact of data types (FP16) and embedding dimensionality, we run those microbenchmarks on the 4th Generation Intel Xeon Scalable processor (Sapphire Rapids) in a VM on Google \texttt{c3-highcpu-4} instance.

\input{06-evaluation/cpu_types_card_graph}

\subsubsection{Data Type and Tensor Formulation}

We analyze the impact of the data type and algorithm formulation on the execution time. We compare the standard nested-loop join implementation versus tensor formulation. We focus on the execution time taken to compute only the cosine distance and isolate the execution time from retrieving the result after applying the cosine distance threshold predicate. 
We fix the embedding vector size to 256 and vary the data type sizes: 16-bit floating point (FP16), 32-bit floating point (FP32), and 64-bit floating point (FP64). We indicate the tensor formulation of cosine distance using 32- and 64-bit data types over CPU as TF32 and TF64, respectively. We run the microbenchmarks over a single CPU core (Sapphire Rapids). We vary the input relation sizes from 5k x 5k (25k comparisons), 10k x 10k (100k comparisons), and 20k x 20k (400k comparisons) and have the embeddings prefetched in memory, with results in \autoref{fig:cpuTypeCardinality}.

\autoref{fig:cpuTypeCardinalityNLJ} shows the scalability of the NLJ cost formulation, which scales linearly with the number of comparisons (quadratically with the input relation size), validating the cost model formulation with prefetching. By reducing the data type precision (hardware supported), FP32 to FP64 sees close to 2x improvement, while FP32 to FP16 further improves the execution time.
\autoref{fig:cpuTypeCardinalityTensor} shows the tensor join formulation against the fastest (FP16) NLJ formulation execution time (same FP16 bar as in \autoref{fig:cpuTypeCardinalityNLJ} for cross-reference). It demonstrates that a correct, cache and instruction-efficient linear algebra matrix join formulation can be 4x faster than a traditional relational Nested-Loop Join, despite having a 4x larger data type footprint (TF64 vs. FP16) and the importance of physical optimizations.


We are further interested in the impact of the embedding vector size on the execution time, on both tensor and NLJ formulations, as in \autoref{fig:cpuModelCardinality}. The vector dimensionality impacts the execution time linearly by increasing the per-vector computation size. 
\autoref{fig:cpuModelCardinalityTensor} demonstrates the tensor formulation scalability. In contrast, \autoref{fig:cpuModelCardinalityNLJ} shows the NLJ formulation over different data types - note that the FP16 bar is the same across both figures to provide a cross-reference point.

Selecting the correct logical and physical optimization can result in orders of magnitude performance differences on the same input data size, indicating the importance of fine-tuned and holistic optimizations and trade-offs between exact model accuracy, both in vector embedding size and representing data type size.


\input{06-evaluation/cpu_types_model_graph}


%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Parallelization and Vectorization}

Next, we demonstrate the scalability of CPU execution and physical and logical optimizations. 
First, we investigate the impact of SIMD vectorization (\autoref{fig:cpuScalabilitySIMD}). 
We enable hyperthreading (24 physical, 48 logical cores), affinitize threads to cores (2 threads will run on 1 physical core, 4 on 2, etc.), and run the NLJ formulation of 10k x 10k relation size input, with 32-bit, 100-dimensional embeddings. 
The processor has AVX-512 registers that can simultaneously fit up to 16 32-bit floating-point values. 
The average improvement is 5.36x, indicating non-computational overheads during vectorization but improved execution time using available hardware intrinsics.

\input{06-evaluation/cpu_simd_scalability}


Next, we use two strategies to investigate the effect of affinitizing threads to cores (\autoref{fig:cpuScalabilityAff}). First, we assign the physical cores to the thread pool, followed by hyper-threads. Second, we affinitize threads and hyper-threads to cores (2 threads will run on 1 physical core, 4 on 2, until 24 cores/48 threads). While affinitized strategy scales with added cores, physical cores scale faster, and hyper-threads do not contribute to improved execution time. This corroborates that dense vector linear algebra is computationally heavy, and physical cores cannot simultaneously benefit from scheduling a hyper-thread. 
At the shift from physical to added logical cores, we see an increase in the physical$\rightarrow$HTs strategy due to data-parallel execution at 28 threads, as 28 partitions were assigned to 24 physical cores, creating 4 stragglers. 
Finally, using all the available resources, the result is the same.

\input{06-evaluation/cpu_affinity_scalability}


In \autoref{fig:cpuScalabilityPref}, we show the scalability of model embedding vector prefetching according to the proposed logical optimization (\autoref{sec:logical-optimization}). 
We compare model prefetching over two input relations sized 10k x 10k, and 100k x 100k, which results in $10^{8}$ and $10^{10}$ computations, respectively. Notice the \textit{log}-scale of the figure.
Using the improved NLJ cost model formulation and comparing the execution time between the two input sizes, execution time scales linearly instead of quadratically as in the non-optimized case and by an expected factor of $10^{2}$.

\input{06-evaluation/cpu_prefetch_scalability}



%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{End-to-End Runtime}

\input{06-evaluation/cpu_endtoend}

Finally, we are interested in how context-enhanced relational join performs on the CPU in an end-to-end context-rich join runtime. 
We run the experiments over 100-d, 32-bit embeddings over 48 threads and investigate the impact of physical and logical optimizations using the Nested-Loop Join formulation.

In the first experiment (\autoref{fig:cpuNLJendtoend}), we investigate the effects of input sizes, number of computations, and ordering of input relations of context-enhanced NLJ implementation. 
First, we notice that the execution time scales linearly with the number of computations/operations performed, according to the cost model. 
Second, we validate that to achieve improved execution time due to cache locality, smaller relation should still be the inner loop, as in the traditional nested-loop-join, while using 100-d vectors for cosine distance computation. Despite more expensive per-vector computations, data access patterns still play an important role, impacting our experiment's performance by up to $\sim$35\% (at $10^{10}$ operations).

\input{06-evaluation/cpu_noprefetch_endtoend}

To conclude CPU-based experiments, we evaluate the impact of logical optimization of model prefetching and physical optimization using SIMD in \autoref{fig:cpuNLJendtoendSIMD}. 
We denote with \textit{Prefetch} the cost model that considers prefetching the embeddings as in \autoref{nlj-prefetch}, and use \autoref{nlj-naive} otherwise. 
Not prefetching the embeddings incurs quadratic model access costs validating the cost model, resulting in orders of magnitude slower execution time. 
This emphasizes the importance of analyzing, exposing, and optimizing model-operator interactions.
Despite using the same hardware resources, including separate experiments with and without SIMD, the execution time demonstrates that the main bottleneck is not computational but access-pattern related. With wrong holistic operator formulation, faster hardware may be unable to correct suboptimal formulation, as it may happen with imperative operator specification by a non-expert user.
In this case, the optimal strategy of prefetching the embeddings first and then joining, despite having two separate tasks, allows faster execution time. SIMD instructions improve the execution time 2x, indicating a computational bottleneck that additional hardware instructions reduce, while this is not the case in the non-prefetch, sub-optimal formulation.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% GPU
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{GPU Performance}

We evaluate the performance of context-enhanced operators on the GPU using the tensor join formulation, the impact of data transfers, and end-to-end execution time compared to the CPU execution time using the Nested-Loop Join formulation.

\paragraph{System and Hardware Setup} We implement our benchmarks in a standalone system in Tensorflow on Google Colab Pro using TensorFlow 2.11.0 for high-performance linear algebra framework, using NVIDIA A100-SXM4-40GB GPU. While the program specification is in Python, TensorFlow compiles and executes these operations into an efficient, hardware-conscious runtime.


\subsubsection{GPU Transfers and Batching}
\input{06-evaluation/gpu_transfer_batches_graph}

As GPUs have limited onboard memory, transferring the data from the CPU-local main memory requires maintaining a limited data partition on the GPU side for processing. 
We achieve this using the partitioning of \autoref{eq:decomposition}, and implement dataset batching using TensorFlow Dataset API.
The maximum matrix batch in our experiments is set to 100k x 10k, after which we reach the out-of-memory exception on GPU.

\autoref{fig:gpuTensendtoendBatch} evaluates the impact of batch transfer size using fixed 100k x 100k input relation and the impact of different data type representations. 
When the transfer and data access is the bottleneck, changing the data type to a more compact representation does not improve the performance. It degrades the end-to-end execution time by orders of magnitude if misconfigured.
Increasing the allocation and transfer granularity improves the execution time by orders of magnitude, finally enabling computational improvements using more efficient data representations (TF16, TF32, and TF64) at the memory capacity of the GPU. Optimizing data access and CPU to GPU transfer bottlenecks is crucial to efficiently utilize the GPU and reduce the end-to-end execution time.



\subsubsection{Cosine Distance with Tensor Formulation}
\input{06-evaluation/gpu_types_card_graph}

Next, we investigate the tensor join formulation execution time (\autoref{fig:tensor}) on GPU and vary the input relation size over 100-dimensional embeddings, always using a transfer batch size of 100k x 10k. 
The results are in \autoref{fig:gpuCosine} and indicate the scalability of context-rich joins with embeddings using cosine distance using GPU runtimes. At the same time, there is an execution time difference between FP16, FP32, and FP64 data types that do not ideally scale due to transfer bottlenecks. Still, FP16 execution time is unexpectedly similar to FP32, indicating transfer bottlenecks and possible sub-optimal support for linear algebra operations over half-precision types—nonetheless, GPU execution processes 1Mx1M input in up to 16 seconds.

\subsubsection{End-to-End Runtime}
\input{06-evaluation/gpu_endtoend} Finally, in \autoref{fig:gpucpuNLJendtoend}, we compare the GPU end-to-end join execution time, as in \autoref{fig:tensor}, and compare it with CPU NLJ formulation with prefetching on CPU using 48 threads. We set embeddings to 100 dimensions. There are now added operations to the cosine distance computation: inequality computation and extracting the fields that satisfy the condition, which increases the GPU execution time compared to \autoref{fig:gpuCosine}, linearly scaling at the largest inputs (10x). Different input sizes can equally be considered a microbenchmark on the impact of filter operator pushdown. Faster memory and massive parallelism of GPUs provide several orders of magnitude faster context-rich joins, despite added transfer time, proving GPUs to be a hardware runtime of choice for using tensor-based join formulation. 

\paragraph{Takeaway}
Our experiments demonstrate the importance of holistic optimizations, spanning logical, physical, and hardware optimizations, yielding several orders of magnitude improvements in execution time. 
Such optimizations are non-trivial for non-expert users in ad-hoc and complex queries, which motivates systematic integration with existing optimizable algebra. Our case study using the join operator shows that synergetic optimizations allow novel functionality, efficiency, and reduced execution time for context-enhanced relational operators using neural embeddings.



==> 06-evaluation/main-prev.tex <==
\label{sec:evaluation}

We start by demonstrating the functionality of using models as a driver of context-enhanced relational operations through the example of word embeddings. 
We then focus on the main performance evaluation of the proposed logical and physical optimizations, showing that a holistic approach is necessary to obtain a performant join algorithm.

\textbf{System} We implement our prototype operators and evaluation in a standalone system in C++ and use Intel AVX instructions for SIMD execution. Tensor formulation benchmarks use Intel oneAPI Math Kernel Library for CPU-aware and efficient BLAS-based linear algebra operations.

\textbf{Hardware Setup} We run the end-to-end and scalability experiments on a two-socket Intel Xeon Gold 5118 CPU (2 x 12-core, 48 threads) and 384GB of RAM. All experiments are with in-memory data; experiments with synthetic data use the same random number generator seed for reproducibility. 
%To evaluate the impact of half-precision floating point (FP16) on the processing cost, we run those microbenchmarks on the 4th Generation Intel Xeon Scalable processor (Sapphire Rapids) in a VM on Google \texttt{c3-highcpu-4} instance.


\subsection{Enhancing Operator Context via Word Embeddings}
In our study, we use the example of word embeddings that transform input strings into high-dimensional vectors. 
We show the context-awareness functionality that word embeddings allow and note that embedding models can be fine-tuned and replaced to support different notions of similarity. 
Conversely, there are embedding models to support different data modalities. 
Still, the intermediate data representation of an embedding is a context-free vector that operators process independently of the particular model, on top of which we base our analysis.
The proposed optimizations of our approach are independent by design and principled in approach due to the separation of concerns between the model, which produces vectors, and the operator performing the join over context-free vectors.

\textbf{Embedding Model}
%We use FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17} word embedding model, which allows out-of-vocabulary embeddings and retrieving in-vocabulary embeddings from a hash-table structure. 
We use FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17, DBLP:conf/naacl/EdizelPBFGS19} as a model ($\mu$) for string embeddings, which has the desirable properties that it can be trained and adapted to the context, it supports out of vocabulary word embedding and is resilient to misspellings. A context-aware operator is supplemented with an embedding model. In this case, when an operator receives strings, it embeds them using FastText and then performs the requested processing in the vector domain. 

\textbf{Dataset}
We train a 100-dimension embedding model over a subset of Wikipedia dataset~\cite{wiki}, cleaned of stopwords, using a subset of 1M strings from the dataset to test the similarity using the model.
We show the nearest vectors to sample words as the strings are embedded into a high-dimensional vector space. We then decode the vectors back into string and present sample semantic matches in \autoref{tab:sem_example}. The model has learned semantics and context from the Wikipedia dataset. To fine-tune the model, it is possible to specialize the embedding models with other domain-specific datasets. 


\begin{table}[hb]% h asks to places the floating element [h]ere.
  \caption{Semantic Matching using FastText trained on Wikipedia dataset, 100-D embeddings, sample words.}
  \label{tab:sem_example}
  \begin{tabularx}{\linewidth}{p{0.12\linewidth}  p{0.82\linewidth} }
    \toprule
    Word & Top-15 Model Matches\\
    \midrule
    dbms & rdbms, nosql, dbmss, postgresql, rdbmss, sql, dbmses, sqlite, dataflow, ordbms, oodbms, couchdb, mysql, ldap, oltp\\
    \hline
    postgres & postgre, postgresql, openvt, dbms, rdbmss, sqlite, dbmss, odbc, backend, rdbms, rdbmses, postgis, openvp, couchdb, mysql\\
    \hline
    animal & animals, felines, human, bovines, equines, dogs, nonhuman, ferrets, rabbits, chickens, anthropods, bovine, anthropod, mammal, equine\\
    \hline
     dog & dogs, poodle, doberman, sheepdog, puppies, dachshund, hound, bullmastiff, retriever, pinschers, dobermans, puppy, bullmastiffs, chickenhound, dachshunds\\
    \hline
    clothes & dresses, clothing, garments, underwear, bedclothes, undergarments, towels, underwears, scarves, shoes, nightgowns, clothings, bathrobes, underclothes\\
  \bottomrule
\end{tabularx}
\end{table}


It is important to mention that models allow automated semantic matching, and the strings are not materialized or retrieved during operations in an intermediate step. The computation entirely happens on embedded data, and only positive matches are retrieved. It is possible to decode the embeddings, for example, based on their offset in the input relation and processing the embedding using standard encoder-decoder model architecture.

This model detected synonyms, semantic and related matches, and plural forms of the words without external user specification. The only parameter in the case of a join with cosine distance would be a single threshold parameter. This allows relational operators normally operating over sample strings (i.e., Word column in \autoref{tab:sem_example}) to perform matches with strings on the right in the embedding domain without humans in the loop or experts that would create and specify strict rules. Such models can work by providing positive match examples that could infer the correct cosine distance threshold parameter.


%More expensive models, online, bert, future work! no standardized benchmark, but the benefit is recognized, and we do not claim the benefits of embeddings, but formalize how they should interact. still, we provide a preview, also available for other multi-modal data. Open source and closed-source models, cost analysis. Dimensions can also change, but usually vary from X to Y, but the main benefit is that the data type itself is immutable (tensors), therefore the analysis.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CPU
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% alternatively just have performance and subsubsections
%%
%% 1. Hardware-conscious vector processing
%% 2. Optimizing NLJ with model prefetching 
%% 3. Tensor join formulation 
%% 4. Point versus batched requests
%% 5. Bounding the memory footprint
%%
\subsection{Hardware-Conscious Vector Processing}
We first evaluate the impact of logical and physical optimizations on the execution times.


\input{06-evaluation/new_cpu_approaches.tex}


%\input{06-evaluation/new_cpu_approaches_perD.tex}

%\input{06-evaluation/new_cpu_gemm_batch_perD.tex}


\input{06-evaluation/new_cpu_gemm_batch.tex}

%\input{06-evaluation/cpu_types_card_graph}
%\subsubsection{Data Type and Tensor Formulation}

% We analyze the impact of the data type and algorithm formulation on the execution time. We compare the standard nested-loop join implementation versus tensor formulation. We focus on the execution time taken to compute only the cosine distance and isolate the execution time from retrieving the result after applying the cosine distance threshold predicate. 
% We fix the embedding vector size to 256 and vary the data type sizes: 16-bit floating point (FP16), 32-bit floating point (FP32), and 64-bit floating point (FP64). We indicate the tensor formulation of cosine distance using 32- and 64-bit data types over CPU as TF32 and TF64, respectively. We run the microbenchmarks over a single CPU core (Sapphire Rapids). We vary the input relation sizes from 5k x 5k (25k comparisons), 10k x 10k (100k comparisons), and 20k x 20k (400k comparisons) and have the embeddings prefetched in memory, with results in \autoref{fig:cpuTypeCardinality}.

% \autoref{fig:cpuTypeCardinalityNLJ} shows the scalability of the NLJ cost formulation, which scales linearly with the number of comparisons (quadratically with the input relation size), validating the cost model formulation with prefetching. By reducing the data type precision (hardware supported), FP32 to FP64 sees close to 2x improvement, while FP32 to FP16 further improves the execution time.
% \autoref{fig:cpuTypeCardinalityTensor} shows the tensor join formulation against the fastest (FP16) NLJ formulation execution time (same FP16 bar as in \autoref{fig:cpuTypeCardinalityNLJ} for cross-reference). It demonstrates that a correct, cache and instruction-efficient linear algebra matrix join formulation can be 4x faster than a traditional relational Nested-Loop Join, despite having a 4x larger data type footprint (TF64 vs. FP16) and the importance of physical optimizations.


% We are further interested in the impact of the embedding vector size on the execution time, on both tensor and NLJ formulations, as in \autoref{fig:cpuModelCardinality}. The vector dimensionality impacts the execution time linearly by increasing the per-vector computation size. 
% \autoref{fig:cpuModelCardinalityTensor} demonstrates the tensor formulation scalability. In contrast, \autoref{fig:cpuModelCardinalityNLJ} shows the NLJ formulation over different data types - note that the FP16 bar is the same across both figures to provide a cross-reference point.

% Selecting the correct logical and physical optimization can result in orders of magnitude performance differences on the same input data size, indicating the importance of fine-tuned and holistic optimizations and trade-offs between exact model accuracy, both in vector embedding size and representing data type size.


% \input{06-evaluation/cpu_types_model_graph}


%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Parallelization and Vectorization}

Next, we demonstrate the scalability of CPU execution and physical and logical optimizations. 
First, we investigate the impact of SIMD vectorization (\autoref{fig:cpuScalabilitySIMD}). 
We enable hyperthreading (24 physical, 48 logical cores), affinitize threads to cores (2 threads will run on 1 physical core, 4 on 2, etc.), and run the NLJ formulation of 10k x 10k relation size input, with 32-bit, 100-dimensional embeddings. 
The processor has AVX-512 registers that can simultaneously fit up to 16 32-bit floating-point values. 
The average improvement is 5.36x, indicating non-computational overheads during vectorization but improved execution time using available hardware intrinsics.

\input{06-evaluation/cpu_simd_scalability}


Next, we use two strategies to investigate the effect of affinitizing threads to cores (\autoref{fig:cpuScalabilityAff}). First, we assign the physical cores to the thread pool, followed by hyper-threads. Second, we affinitize threads and hyper-threads to cores (2 threads will run on 1 physical core, 4 on 2, until 24 cores/48 threads). While affinitized strategy scales with added cores, physical cores scale faster, and hyper-threads do not contribute to improved execution time. This corroborates that dense vector linear algebra is computationally heavy, and physical cores cannot simultaneously benefit from scheduling a hyper-thread. 
At the shift from physical to added logical cores, we see an increase in the physical$\rightarrow$HTs strategy due to data-parallel execution at 28 threads, as 28 partitions were assigned to 24 physical cores, creating 4 stragglers. 
Finally, using all the available resources, the result is the same.

\input{06-evaluation/cpu_affinity_scalability}


In \autoref{fig:cpuScalabilityPref}, we show the scalability of model embedding vector prefetching according to the proposed logical optimization (\autoref{sec:logical-optimization}). 
We compare model prefetching over two input relations sized 10k x 10k, and 100k x 100k, which results in $10^{8}$ and $10^{10}$ computations, respectively. Notice the \textit{log}-scale of the figure.
Using the improved NLJ cost model formulation and comparing the execution time between the two input sizes, execution time scales linearly instead of quadratically as in the non-optimized case and by an expected factor of $10^{2}$.

\input{06-evaluation/cpu_prefetch_scalability}



%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{End-to-End Runtime}

\input{06-evaluation/cpu_endtoend}

Finally, we are interested in how context-enhanced relational join performs on the CPU in an end-to-end context-rich join runtime. 
We run the experiments over 100-d, 32-bit embeddings over 48 threads and investigate the impact of physical and logical optimizations using the Nested-Loop Join formulation.

In the first experiment (\autoref{fig:cpuNLJendtoend}), we investigate the effects of input sizes, number of computations, and ordering of input relations of context-enhanced NLJ implementation. 
First, we notice that the execution time scales linearly with the number of computations/operations performed, according to the cost model. 
Second, we validate that to achieve improved execution time due to cache locality, smaller relation should still be the inner loop, as in the traditional nested-loop-join, while using 100-d vectors for cosine distance computation. Despite more expensive per-vector computations, data access patterns still play an important role, impacting our experiment's performance by up to $\sim$35\% (at $10^{10}$ operations).

\input{06-evaluation/cpu_noprefetch_endtoend}

To conclude CPU-based experiments, we evaluate the impact of logical optimization of model prefetching and physical optimization using SIMD in \autoref{fig:cpuNLJendtoendSIMD}. 
We denote with \textit{Prefetch} the cost model that considers prefetching the embeddings as in \autoref{nlj-prefetch}, and use \autoref{nlj-naive} otherwise. 
Not prefetching the embeddings incurs quadratic model access costs validating the cost model, resulting in orders of magnitude slower execution time. 
This emphasizes the importance of analyzing, exposing, and optimizing model-operator interactions.
Despite using the same hardware resources, including separate experiments with and without SIMD, the execution time demonstrates that the main bottleneck is not computational but access-pattern related. With wrong holistic operator formulation, faster hardware may be unable to correct suboptimal formulation, as it may happen with imperative operator specification by a non-expert user.
In this case, the optimal strategy of prefetching the embeddings first and then joining, despite having two separate tasks, allows faster execution time. SIMD instructions improve the execution time 2x, indicating a computational bottleneck that additional hardware instructions reduce, while this is not the case in the non-prefetch, sub-optimal formulation.


\subsection{Optimizing NLJ with prefetching and batching}
\textcolor{red}{expand and explain}

\subsection{Tensor join formulation}
\textcolor{red}{expand and explain}

\subsection{Bounding the memory footprint}
\textcolor{red}{expand and explain}

\subsection{Point versus batched requests}
\textcolor{red}{expand and explain}

\input{06-evaluation/new_tensor_nlj.tex}

\input{06-evaluation/new_memory_batch10k.tex}

\input{06-evaluation/new_memory_batch100k.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tensor formulation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{GPU Performance}

% We evaluate the performance of context-enhanced operators on the GPU using the tensor join formulation, the impact of data transfers, and end-to-end execution time compared to the CPU execution time using the Nested-Loop Join formulation.

% \paragraph{System and Hardware Setup} We implement our benchmarks in a standalone system in Tensorflow on Google Colab Pro using TensorFlow 2.11.0 for high-performance linear algebra framework, using NVIDIA A100-SXM4-40GB GPU. While the program specification is in Python, TensorFlow compiles and executes these operations into an efficient, hardware-conscious runtime.


% \subsubsection{GPU Transfers and Batching}
% \input{06-evaluation/gpu_transfer_batches_graph}

% As GPUs have limited onboard memory, transferring the data from the CPU-local main memory requires maintaining a limited data partition on the GPU side for processing. 
% We achieve this using the partitioning of \autoref{eq:decomposition}, and implement dataset batching using TensorFlow Dataset API.
% The maximum matrix batch in our experiments is set to 100k x 10k, after which we reach the out-of-memory exception on GPU.

% \autoref{fig:gpuTensendtoendBatch} evaluates the impact of batch transfer size using fixed 100k x 100k input relation and the impact of different data type representations. 
% When the transfer and data access is the bottleneck, changing the data type to a more compact representation does not improve the performance. It degrades the end-to-end execution time by orders of magnitude if misconfigured.
% Increasing the allocation and transfer granularity improves the execution time by orders of magnitude, finally enabling computational improvements using more efficient data representations (TF16, TF32, and TF64) at the memory capacity of the GPU. Optimizing data access and CPU to GPU transfer bottlenecks is crucial to efficiently utilize the GPU and reduce the end-to-end execution time.



% \subsubsection{Cosine Distance with Tensor Formulation}
% \input{06-evaluation/gpu_types_card_graph}

% Next, we investigate the tensor join formulation execution time (\autoref{fig:tensor}) on GPU and vary the input relation size over 100-dimensional embeddings, always using a transfer batch size of 100k x 10k. 
% The results are in \autoref{fig:gpuCosine} and indicate the scalability of context-rich joins with embeddings using cosine distance using GPU runtimes. At the same time, there is an execution time difference between FP16, FP32, and FP64 data types that do not ideally scale due to transfer bottlenecks. Still, FP16 execution time is unexpectedly similar to FP32, indicating transfer bottlenecks and possible sub-optimal support for linear algebra operations over half-precision types—nonetheless, GPU execution processes 1Mx1M input in up to 16 seconds.

% \subsubsection{End-to-End Runtime}
% \input{06-evaluation/gpu_endtoend} Finally, in \autoref{fig:gpucpuNLJendtoend}, we compare the GPU end-to-end join execution time, as in \autoref{fig:tensor}, and compare it with CPU NLJ formulation with prefetching on CPU using 48 threads. We set embeddings to 100 dimensions. There are now added operations to the cosine distance computation: inequality computation and extracting the fields that satisfy the condition, which increases the GPU execution time compared to \autoref{fig:gpuCosine}, linearly scaling at the largest inputs (10x). Different input sizes can equally be considered a microbenchmark on the impact of filter operator pushdown. Faster memory and massive parallelism of GPUs provide several orders of magnitude faster context-rich joins, despite added transfer time, proving GPUs to be a hardware runtime of choice for using tensor-based join formulation. 

% \paragraph{Takeaway}
% Our experiments demonstrate the importance of holistic optimizations, spanning logical, physical, and hardware optimizations, yielding several orders of magnitude improvements in execution time. 
% Such optimizations are non-trivial for non-expert users in ad-hoc and complex queries, which motivates systematic integration with existing optimizable algebra. Our case study using the join operator shows that synergetic optimizations allow novel functionality, efficiency, and reduced execution time for context-enhanced relational operators using neural embeddings.



==> 07-related-work/main-old.tex <==
\label{sec:related-work}
This section outlines the related work and compares and places our approach in the rich design space of prior research.


\subsection{ML for DB}
Machine learning for databases has been a hot topic of research where structural components of DBMS get enhanced using findings from the ML community. 
Learned indexes~\cite{DBLP:conf/sigmod/KraskaBCDP18} avoid data structure traversal by learning the data distribution information and optimizing data access. 
More holistically, using sum-product networks allows for model-driven approximate query processing~\cite{DBLP:journals/pvldb/HilprechtSKMKB20}. 
From a systems perspective, using tensor processing frameworks for traditional relational processing has also recently been proposed~\cite{DBLP:journals/corr/abs-2211-02753}.

Our approach is similar as we propose using ML embedding models to provide context to data traditionally opaque to relational DBMS. 
We propose a general framework for extending and analyzing relational operators using novel model-database interactions.


\subsection{DB for ML}
On the other hand, databases for machine learning focus on applying or integrating machine learning components with systems. 
More broadly, frameworks such as Tensorflow~\cite{abadi2016tensorflow} or Pytorch~\cite{paszke2019pytorch} are efficient, hardware-conscious dataflow engines.
There has been recent work on developing vector-specialized databases~\cite{DBLP:journals/tbd/JohnsonDJ21} typically based on indexes for efficient high-dimensional similarity search~\cite{DBLP:conf/sigmod/WangYGJXLWGLXYY21}. 
Still, such engines often lack a DBMS's expressiveness, functionality, and analytical operations for more complex data analysis, which would force users to write imperative code to integrate different siloed system components. We propose holistic optimizations and functionality built on, compatible with, and extending relational DBMS.

There has also been work on bringing machine learning training and inference closer to analytical engines~\cite{DBLP:journals/pvldb/HellersteinRSWFGNWFLK12}, including neural networks and deep learning operations~\cite{DBLP:conf/icde/LinWZDLC22}.
Such approaches are compatible with our work, as they allow exposing data structures and operations between models and relational operators in a unified framework. Therefore, such system approaches would benefit future work topics, such as cost-driven query optimization.


\subsection{String Similarity Joins}
In our paper, we have analyzed a join operator that functionally belongs to approximate string similarity joins.
Traditional string similarity techniques require exact similarity specification using edit distance or q-grams as token-based string similarity~\cite{10.5555/645927.672200}. Similarly, locality-sensitive hashing techniques~\cite{10.1145/3292500.3330853} allow approximate string similarity joins. These approaches are adequate for finding misspellings and limited token-based differences. 

In contrast, we propose using word embedding models capable of identifying misspellings, different tenses, and semantic similarity based on training and fine-tuning training dataset and parameters~\cite{DBLP:journals/tacl/BojanowskiGJM17, DBLP:conf/naacl/EdizelPBFGS19}. Through the separation of concerns, from the perspective of DBMS, string similarity join has a tensor-based input with cosine distance and threshold as parameters. At the same time, the embedding model handles the string semantics and context and transforms the input into context-free embeddings for RDBMS to process.

\subsection{Representation Learning}
The significant body of work in representation learning is the key enabler of context-rich relational operators. 
It allows for transforming the human-centric, context-rich data representations into machine-centric formats amenable to automated processing.
We combine ML-based embedding models with relational operators and analyze end-to-end interactions, from logical to physical optimizations. Such models allow masking and transforming contextual data into embeddings as ubiquitous data representations that can be processed by extending RDBMS with tensor-based operators.

While we focused on string-based similarity using FastText~\cite{DBLP:journals/tacl/BojanowskiGJM17, DBLP:conf/naacl/EdizelPBFGS19}, there are other embedding models designed for natural language processing such as word2Vec~\cite{DBLP:journals/corr/abs-1301-3781}, BERT~\cite{DBLP:conf/naacl/DevlinCLT19}, or GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20}.

Furthermore, a rich research area in machine learning drives embedding models that support other context-rich data formats, equally transforming the input into context-free embeddings. Enabling multi-modality through model-operator interactions in a topic of future research, where models such as ResNet~\cite{DBLP:conf/cvpr/HeZRS16} can be used for images or PANNs~\cite{DBLP:journals/taslp/KongCIWWP20} for audio processing. Models trained on web-scale data exist as Foundation Models~\cite{DBLP:journals/corr/abs-2108-07258}, that can be re-trained and adapted for a specific task and dataset.


==> 08-conclusion/main-old.tex <==
\label{sec:conclusion}
%conclusion
Data management systems aim to support and adapt to modern data processing requirements and adopt innovations. 
With strong results in automating context-rich processing from the machine learning community, such individual components would require imperative integration in complex analytical data pipelines.
Our context-rich operators integrate embedding models with relational operators based on the key observation of separation of concerns. 
Embedding models are designed to handle context, while RDBMS needs to provide a declarative context-free interface that allows logical and physical optimizations of the interactions between operators and models.
With the common tensor data representation, we analyze the behavior of a join operator and propose relational algebra extensions, logical and physical optimizations, and introduce optimizations for execution on CPUs and GPUs.
We evaluate our cost model and show the impact holistic optimizations have on the execution time, resulting in orders of magnitude differences across logical, physical, and hardware optimizations.

%future directions
We propose analyzing and optimizing model-relational interactions with the aim of context-rich processing, which opens future research questions. 
With many context-rich data unsuitable for DBMS, our approach allows a generalized way to allow some multi-modality features. 
Still, various data formats and models may have different computational or data access tradeoffs that impact the performance of an operator.
Similarly, unifying cost- and rule-based query optimization under a single framework would require systematic model evaluation cost estimation.
From the hardware perspective, accelerators such as TPUs or heterogeneous computation platforms present complex environments with many interactions and considerations, such as model and operator placement, load balancing, and resource scheduling. 
It is also crucial to analyze storage hierarchy, caching, and data structures for tensor-relational data.
Finally, developing benchmarks for multi-modal and context-rich data would allow systematic comparison of future systems.

%model-relational analytics
%if external models/price used, then storing and caching makes sense
%mostly for the mismatch between analytical and model part, if using all on local infrastructure,
% https://medium.com/@nils_reimers/openai-gpt-3-text-embeddings-really-a-new-state-of-the-art-in-dense-text-embeddings-6571fe3ec9d9
%or price mismatch and very high latency with external services.
%https://openai.com/pricing
%approximate joins, or partitioning strategies for data structures (e.g. opening the interaction)
%still, with more fine-tuned models and to control latency, data, performance, models will become part of analytics.

